Eliciting Better Multilingual Structured Reasoning from LLMs through Code

The development of large language models (LLM) has shown progress on reasoning, though studies have largely considered either English or simple reasoning tasks. To address this, we introduce a multilingual structured reasoning and explanation dataset, termed xSTREET, that covers four tasks across six languages. xSTREET exposes a gap in base LLM performance between English and non-English reasoning tasks. We then propose two methods to remedy this gap, building on the insight that LLMs trained on code are better reasoners. First, at training time, we augment a code dataset with multilingual comments using machine translation while keeping program code as-is. Second, at inference time, we bridge the gap between training and inference by employing a prompt structure that incorporates step-by-step code primitives to derive new facts and find a solution. Our methods show improved multilingual performance on xSTREET, most notably on the scientific commonsense reasoning subtask. Furthermore, the models show no regression on non-reasoning tasks, thus demonstrating our techniques maintain general-purpose abilities.

==> arc_ar_ex.tex <==
\begin{table*}[ht!]
\centering
\tiny
\setlength{\tabcolsep}{4pt}

\begin{tabularx}{\linewidth}{lX} \toprule
\Sim\ code input & 
facts = {[} '\RL{القمر هو الجسم السماوي الأقرب إلى الأرض من الشمس}',\newline '\RL{جاذبية القمر على محيطات الأرض تتسبب في المد والجزر}',\newline  '\RL{جاذبية الشمس على محيطات الأرض تتسبب في المد والجزر}',\newline \RL{'كلما انخفضت المسافة من جسم ما، تزداد قوة الجاذبية على هذا الجسم}'{]}\newline  question = '\RL{يتأثر المد والجزر على الأرض بالقمر أكثر من الشمس لأن القمر}' \newline  choices = \{'A': '\RL{أكثر إشراقًا من الشمس.}',  'B': '\RL{أكبر من الأرض.}',  'C': '\RL{أبرد من الأرض.}',  'D': '\RL{أقرب من الشمس.}'\}\newline  answer = None\newline \# call select\_facts and infer\_new\_fact until answer is set\newline selected = select\_facts(facts) \#  "
\\ \midrule
Linearized input & QUESTION = 
sent1:\RL{القمر هو الجسم السماوي الأقرب إلى الأرض من الشمس}
 sent2:\RL{جاذبية القمر على محيطات الأرض تتسبب في المد والجزر} 
 sent3:\RL{جاذبية الشمس على محيطات الأرض تتسبب في المد والجزر} 
 sent4:\RL{كلما انخفضت المسافة من جسم ما، تزداد قوة الجاذبية على هذا الجسم} 
 sent5:\RL{يتأثر المد والجزر على الأرض بالقمر أكثر من الشمس لأن القمر}
 sent6: A) \RL{أكثر إشراقًا من الشمس.} 
 sent7: B) \RL{أكبر من الأرض.} 
 sent8: C) \RL{أبرد من الأرض.} 
 sent9: D) \RL{أقرب من الشمس.} \newline  PROOF = \\ \bottomrule
\end{tabularx}

\begin{tabularx}{\textwidth}{lXX} \toprule
& Gold & GPT-3  \\ \midrule
    \rotatebox{90}{\hspace{-10em} \Sim\ code output} 
    & {[}facts{[}0], facts{[}3]]

new\_fact = infer\_new\_fact(selected) \# '\RL{قوة جاذبية القمر على الأرض أكبر من جاذبية الشمس على الأرض}'

 
is\_solved(new\_fact, choices) \# False

facts.append(new\_fact)

 

selected = select\_facts(facts) \# {[}facts{[}1{]}, facts{[}2{]}, facts{[}4{]}{]}

new\_fact = infer\_new\_fact(selected) \# '\RL{جاذبية القمر على الأرض لها تأثير على ظاهرة المد والجزر بشكل أكبر من جاذبية الشمس}' 

is\_solved(new\_fact, choices) \# False

facts.append(new\_fact)

 

selected = select\_facts(facts) \# {[}facts{[}5{]}{]}

new\_fact = infer\_new\_fact(selected) \# 'The answer is D'

is\_solved(new\_fact, choices) \# True

answer = make\_choice(new\_fact, choices) \# '\textcolor{OliveGreen}{D}'",
    
    & [facts[0], facts[1], facts[2], facts[3]]

new\_fact = infer\_new\_fact(selected) \# '\RL{جاذبية القمر على الأرض تتسبب في المد والجزر بسبب قربه من الأرض}'


is\_solved(new\_fact, choices) \# False\newline facts.append(new\_fact)

 

selected = select\_facts(facts) \# [facts[4]]

new\_fact = infer\_new\_fact(selected) \# 'The answer is D'

is\_solved(new\_fact, choices) \# True

answer = make\_choice(new\_fact, choices) \# '\textcolor{OliveGreen}{D}'
    \\ \midrule   
    \rotatebox[origin=c]{90}{linearized output} & sent1 \& sent4 -> int1: \RL{قوة جاذبية القمر على الأرض أكبر من جاذبية الشمس على الأرض};  sent2 \& sent3 \& int1 -> int2: \RL{جاذبية القمر على الأرض لها تأثير على ظاهرة المد والجزر بشكل أكبر من جاذبية الشمس};  int2 -> int3: The answer is D);
    &  sent1 \& sent2 -> int1: \RL{القمر هو الجسم السماوي الأقرب إلى الأرض من الشمس ويسبب المد والجزر};  sent3 \& sent4 -> int2: \RL{جاذبية الشمس تسبب المد والجزر على الأرض};  sent5 \& sent6 -> int3: \RL{القمر يسبب المد والجزر أكثر من الشمس لأنه أكثر إشراقًا};  int3 -> int4: The answer is \textcolor{BrickRed}{A}
    \\ \bottomrule
\end{tabularx}
\caption{Case study for a ARC entry, in Arabic. The correct answer is `D' (in green). Only GPT-3 with \Sim\ prompts gets it correct.}
\label{tab:arc_ar_study}
\end{table*}

